Computing in Operations Research using Julia

The state of numerical computing is currently characterized by a divide between highly efficient yet typically cumbersome low-level languages such as C, C++, and Fortran and highly expressive yet typically slow high-level languages such as Python and MATLAB. This paper explores how Julia, a modern programming language for numerical computing which claims to bridge this divide by incorporating recent advances in language and compiler design (such as just-in-time compilation), can be used for implementing software and algorithms fundamental to the field of operations research, with a focus on mathematical optimization. In particular, we demonstrate algebraic modeling for linear and nonlinear optimization and a partial implementation of a practical simplex code. Extensive cross-language benchmarks suggest that Julia is capable of obtaining state-of-the-art performance.

==> parallel.tex <==
\section{Parallel and distributed computing}
\label{sec:Parallel}

The use of parallel computing is increasingly important for improving the time to solution of numerical algorithms. The goal of this section is to provide a case study of using the built-in parallel computing features of Julia to implement a nontrivial decomposition algorithm. While similar capabilities are accessible from other high-level languages, we will illustrate how the design of Julia can greatly facilitate the implementation.

\subsection{Cutting-plane algorithm for nonsmooth convex optimization}
A \textit{subgradient} of a convex function $f : \mathbb{R}^r \to \mathbb{R}$ at a point $x'$ is a vector $g$ such that for all $x \in \mathbb{R}^r$,
\[
    f(x) \ge f(x') + g^T(x-x').
\]

Given a set of subgradients $g_1,\ldots,g_k$ at corresponding points $x^1,\ldots,x^k$, it follows that the \textit{model} function
\begin{equation}\label{eq:mod}
    m_f^k(x) = \max_{i=1,\ldots,k}\{f(x^i) + g_i^T(x-x^i)\}
\end{equation}

is a global underestimator of $f$. This model function is the basis for the classical \textit{cutting-plane} algorithm for minimizing a sum of convex functions $\sum_{j=1}^n f_j(x)$; the algorithm chooses trial points (iterates) by minimizing the model functions and then updating the models with new subgradients. The high-level form of the algorithm may be described as follows:

\begin{algorithm}[h]\small
\caption{Cutting plane algorithm}\label{algserial}
\begin{algorithmic}[1]
\State $k \leftarrow 1$, initialize $x^1$
\Repeat
\For{$j=1,\ldots,n$}
\State Compute function value and subderivative $(f_j(x^k),g_k)$ at $x^k$.
\EndFor
\State $x^{k+1} \leftarrow \operatorname{argmin}_x \sum_{j=1}^n m^k_{f_j}(x)$, with $m^k_{f_j}(x)$ defined by \eqref{eq:mod}
\State $k \leftarrow k + 1$
\Until{convergence}
\end{algorithmic}
\end{algorithm}

The general computational pattern above applies to many classical decomposition methods in optimization, including Benders decomposition, column generation, and Lagrangian relaxation (also known as dual decomposition). Advanced variants, such as bundle methods, also follow the same pattern~\cite[]{LagrangianRelaxation}. Readers are referred to~\cite{HiriartLemarechal93book2} for a thorough introduction.

\subsection{Asynchronous variant}

Algorithm~\ref{algserial} exhibits natural scope for parallelism at Lines 3-5, where $n$ independent operations, usually requiring the solution of an optimization problem, are performed. This form of parallelism, performing completely independent operations, is often called \textit{trivial}, and indeed it is straightforward to implement in Julia and in other existing high-level languages.

However, obtaining the ideal parallel speedup, an $m$-fold speedup given $m$ parallel workers, is not so trivial. In the extreme case of $n$ workers, it is seen that a lower bound on the time to execute Lines 3-5 is the \textit{maximum} of the execution times for each value of $j$, not the average. The difference of these two values is a form of \textit{load imbalance} and arises naturally when linear or, worse, mixed-integer subproblems must be solved, and also when the computing resources are shared among multiple users. An additional barrier to parallel speedup is the serial execution bottleneck of Line 6, which requires the solution of a \textit{master} linear program. 

\cite{Linderoth03} studied this issue in the context of solving large-scale two-stage stochastic programming problems and proposed an asynchronous variant of the cutting-plane algorithm in which when a proportion $0 < \alpha \le 1$ of subproblems for a given iterate $x^k$ have been solved, a new iterate is generated (Line 6) by using whatever subgradients are presently available. In other words, one can generate new subproblems to solve without needing to wait for all current subproblems to complete, making the algorithm asynchronous. The algorithm remains convergent, although the total number of iterations may increase. In the following subsection we describe an implementation of this asynchronous method in Julia.

\subsection{Parallel implementation in Julia}
Julia implements \textit{distributed-memory} parallelism based on \textit{one-sided} message passing; distinct processes with separate states push work onto others (via \texttt{remotecall}) and the results are retrieved (via \texttt{fetch}) by the process which requires them. Communication may occur within a single multicore machine or across a network. 

This model of parallelism contrasts with that of MPI, a low-level API for distributed-memory parallelism used in high-performance computing, where, most commonly, both the sending and receiving processes must explicitly participate in \textit{two-sided} communication. Julia does not presently support shared-memory parallelism such as OpenMP. We refer the reader to~\cite{Grama03} for an introduction to the above mentioned parallel computing concepts and APIs. 

The function \texttt{remotecall(id,f,args)} asynchronously runs \texttt{f(args)} on the process with the given \texttt{id} and returns a \texttt{RemoteRef} object. The value of the \texttt{RemoteRef} can be queried with the \textit{blocking} call \texttt{fetch}, waits for the value to be available before returning. This functionality in itself is typical of similar frameworks (see, e.g., \cite{PyMW}); however, two technical features of Julia, coroutines and macros, enhance this low-level functionality for improved ease of use.

Julia implements coroutines (called \textit{tasks}), a form of lightweight cooperative threads. Each task has its own execution context, and control is yielded explicitly; only one task executes simultaneously, and it cannot be interrupted, alleviating the need to use synchronization constructs such as locks. Coroutines date back to~\cite{ConwayCoroutines} and have been implemented in Python~\cite[]{pythoncoroutine} and C++~\cite[]{cppcoroutine}, although without any syntactic integration with the base libraries. In Julia, on the other hand, they are the idiomatic approach to handle asynchronicity, replacing event loops and callbacks.

Macros provide convenient syntactic wrappers around the low-level \texttt{remotecall} and coroutine functionality. As an illustration, we present a (simplified) implementation of the built-in \texttt{pmap(f,lst)} function which applies the function \texttt{f} to each element of the input \texttt{lst} in parallel using dynamic task allocation and returns the result.

\vspace{0.1in}
\begin{MyCode}[fontsize=\small,fontfamily=pcr]
function pmap(f, lst)
    np = nprocs()     # number of processes available
    n = length(lst)
    results = cell(n) # create empty array
    i = 1
    nextidx() = (idx=i; i+=1; return idx) # define local function
    @sync for p in 1:np
        if p == myid(); continue; end
        @async \textbf{begin} 
            \textbf{while true}  
                \textbf{idx = nextidx()}
                \textbf{if idx > n; break; end}
                \textbf{results[idx] = fetch(remotecall(p, f, lst[idx]))}
            \textbf{end}
        \textbf{end}
    end # main task waits here until all tasks complete
    return results
end
\end{MyCode}

Each invocation of the \texttt{@async} macro within the \texttt{for} loop creates a task that runs on the main process (e.g., process 1). The new task is not immediately executed; instead, the next iteration of the \texttt{for} loop proceeds. The body of the task (in bold) is the code block within the \texttt{begin} and \texttt{end} keywords. When tasks are created, the values of variables from the enclosing scope are captured; hence, in each task the local variable \texttt{p} retains its value from when the task was created. Each task feeds work to its assigned process \texttt{p} using \texttt{remotecall}. The call to \texttt{fetch} surrenders control to another task while waiting for the result. Tasks coordinate work through the \texttt{nextidx} function, which is necessary because they cannot directly modify the variable \texttt{i} from the enclosing scope. The \texttt{@sync} macro prevents the main task from proceeding to the \texttt{return} statement before all tasks have completed.

The use of macros, where blocks of code are automatically transformed into the body of a coroutine and variables are captured from the enclosing scope, permits the above compact implementation of this nontrivial computational pattern. This is achieved without any specialized syntax in Julia beyond the standard syntax for macros.

The \texttt{pmap} routine could be used directly to implement the parallel computations in the synchronous version of the cutting-plane algorithm. For the asynchronous version, we can modify the implementation of \texttt{pmap} above in a straightforward manner. Instead of solving a fixed number of subproblems, we maintain a queue among the tasks; when a subproblem completes, its corresponding task performs a check to trigger resolving the master, generating a new iterate, and adding a new set of subproblems to the queue. We provide a sample implementation below.

\vspace{0.1in}
\begin{MyCode}[fontsize=\small,fontfamily=pcr]
function asyncalgo(f, state, queue, isterminated, processresult)
    np = nprocs() 
    @sync for p in 1:np
        if p == myid(); continue; end
        @async \textbf{begin}
            \textbf{while !isterminated(state)}
                \textbf{if length(queue) == 0; yield(); continue; end}
                
                \textbf{# pop subproblem from queue}
                \textbf{subproblem = shift!(queue)}
                \textbf{result = fetch(remotecall(p, f, subproblem))}
                \textbf{processresult(state, queue, subproblem, result)}
            \textbf{end}
        \textbf{end}
    end
    return state
end
\end{MyCode}

The \texttt{asyncalgo} function takes a function \texttt{f}, an initial \texttt{state} object, an initial \texttt{queue} of subproblems, a function \texttt{isterminated}, and a function \texttt{processresult}. In the decomposition algorithm, the function \texttt{f} corresponds to solving a subproblem, and the function \texttt{processresult} updates the problem state and conditionally resolves the master to generate a new set of subproblems to add to the queue, handling the main logic of the asynchronous algorithm. The implementation retains the structure of the \texttt{pmap} function, with the addition of a check to handle the case where the algorithm has not converged but the queue is empty, which may occur if results have not yet returned. In this case, the \texttt{yield} function is called to surrender control from the current task so other tasks may first process their results.

To address the remaining bottleneck of solving the master problem, we can consider dedicating a process to performing this computation while leaving the main process free to continue distributing work. This is achieved essentially by wrapping the relevant code with the appropriate macro.  

\subsection{Numerical experiments}

The asynchronous trust region (ATR) algorithm of~\cite{Linderoth03} was implemented following the above outline, and we take the \texttt{storm} test instance used by the same authors. \texttt{storm} is a two-stage stochastic linear program; with 20,000 scenarios ($n =$ 20,000), it is equivalent to a linear program with 25 million variables, 10 million constraints, and 66 million nonzero entries in its constraint matrix. Table~\ref{tab:parallel} presents numerical results comparing the synchronous and asynchronous implementations executed on the Amazon Elastic Compute Cloud (EC2).

\begin{table}[th]
	\centering
	\caption{Results on Amazon EC2 comparing the asynchronous and synchronous cutting-plane algorithms (with $\alpha = 0.6$ and $\alpha = 1$ respectively) on the \texttt{storm} test problem with $n = 20,000$. Workers correspond to individual \texttt{m1.medium} instances. The master process is run on an \texttt{m3.xlarge} instance. Speed is the average number of subproblems solved per second. Efficiency is calculated as the percent of ideal parallel speedup obtained. Superlinear speedups (\textgreater 100\%) may be explained by timing variability.
 }\label{tab:parallel} 
	\begin{tabular}{lrrrrrrr}
		\toprule
		& \multicolumn{3}{c}{Synchronous} & \multicolumn{3}{c}{Asynchronous} \\
        \cmidrule(l){2-4}\cmidrule(l){5-7}
		No. Workers& Time-to-sol. (s.) & Speed & Efficiency & Time-to-sol. (s.) & Speed & Efficiency \\
		\cmidrule(l){1-1}\cmidrule(l){2-2}\cmidrule(l){3-3}\cmidrule(l){4-4}\cmidrule(l){5-5}\cmidrule(l){6-6}\cmidrule(l){7-7}
        5 & 3,317 & 78 & Baseline & 11,131 & 76 & Baseline\\
        10 & 1,689 & 154 & 98.2\% & 5,252 & 156 & 103.5\%\\
        20 & 843 & 308 & 98.4\% & 2,629 & 313 & 103.7\%\\
        40 & 434 & 599 & 95.6\% & 1,235 & 620 & 102.8\%\\
        80 & 226 & 1150 & 91.8\% & 646 & 1208 & 100.0\%\\ 
	\bottomrule
	\end{tabular}
\end{table}

While the asynchronous version scales nearly perfectly, it requires more iterations to converge, resulting in the synchronous version solving the problem faster overall. This behavior is highly problem dependent and not well studied in the literature, perhaps due to the perceived difficulty of the implementation. 

